Understanding the Capabilities of Large Language Models for Automated Planning

Automated planning is concerned with developing efficient algorithms to generate plans or sequences of actions to achieve a specific goal in a given environment. Emerging Large Language Models (LLMs) can answer questions, write high-quality programming code, and predict protein folding, showcasing their versatility in solving various tasks beyond language-based problems. In this paper, we aim to explore how LLMs can also be used for automated planning. To do so, we seek to answer four key questions. Firstly, we want to understand the extent to which LLMs can be used for plan generation. Secondly, we aim to identify which pre-training data is most effective in facilitating plan generation. Thirdly, we investigate whether fine-tuning or prompting is a more effective approach for plan generation. Finally, we explore whether LLMs are capable of plan generalization. By answering these questions, the study seeks to shed light on the capabilities of LLMs in solving complex planning problems and provide insights into the most effective approaches for using LLMs in this context.

==> content/approach_orig.tex <==
\section{Materials and Methods}

In this section, we describe the generation of the planning dataset and we discuss the difficulty of the planning domains. We also provide an overview of the LLMs being evaluated and the experimental setup for plan generation.

\subsection{Planning Dataset}

The International Planning Competition (IPC) \citep{ipc} is a biennial event that evaluates state-of-the-art automated planning and scheduling systems. New planners and planning domains are released as part of the IPC. We consider six classical planning domains written in PDDL that were part of the IPC to assess planning capabilities in LLMs. We used problem generators that were released for these domains to generate a planning dataset consisting of 18,000 problems for each domain. A random seed was used to generate the problems and further checked to make sure there are no duplicates present in the dataset. The ground truth optimal plans for these problems are generated using the planner FastDownward, firstly presented by~\citep{helmert2006fast},  with A\textsuperscript{*} LM-Cut heuristics \citep{helmert2011lm}. Table \ref{difficulty} lists the planning domains considered in this paper and classifies them into three difficulty classes. Note that this classification is based on the complexity of the problem in terms of state space and branching factor and the planner used to generate optimal plans. Other factors such as observability of the states and concurrency of actions can also be considered but are not in the scope of this paper as we aim to investigate the optimal plan generation capabilities of LLMs.

% The considered planning domains are \texttt{Blocksworld}, \texttt{Ferry}, \texttt{Miconic}, \texttt{Grippers}, \texttt{Tower of Hanoi}, and \texttt{Driverlog}.

\begin{table}
  \caption{Difficulty of planning domains.}
  \label{difficulty}
  \centering
  \begin{tabular}{llp{5cm}p{3cm}}
    \toprule
    Planning Domain & Difficulty & State Space & Branching Factor\\
    \midrule
    \texttt{Ferry} & Easy & $O(2^{n} * 2 * m * n!)$, $n$ is no. of cars, $m$ is no. of locations & $O(n+1)$\\
    \texttt{Blocksworld} & Easy & $O(3^n)$, $n$ is no. of blocks & $O(4n/2 + 1)$\\
    &\\
    \texttt{Miconic} & Medium & $O(n^{(m+1)} * 2^m *m!)$, $n$ is no. of floors, $m$ is no. of passengers & $O(m+1)$\\
    \texttt{Tower of Hanoi} & Medium & $O(3^n)$, $n$ is no. of disks & $O((k-1)k/2)$, $k$ is no. of pegs\\
    \texttt{Grippers} & Hard & $O(2^n * 3^{nr})$, $n$ is no. of balls, $r$ is no. of robots & $O(3nr + r)$\\
    \texttt{Driverlog} & Hard & $O(L^{(D+T+P)} * K^P * D * T * 2^T)$, $L$ is no. of locations, $D$ is no. of drivers, $T$ is no. of trucks, $P$ is no. of packages & $O(L * (D + T + P + DT + TD))$ \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Data Format for Fine-tuning}

%As LLMs that can be fine-tuned \citep{yosinski2014transferable} are limited in the amount of contextual information they can process, the use of PDDL domain and problem files as input sequences for fine-tuning is constrained by their expressivity. 
The fine-tuning process of LLMs is limited in the amount of contextual information they can handle. This constraint affects the use of PDDL domain and problem files as input sequences for fine-tuning because they may not be expressive enough to provide the necessary context for the model.
To address this limitation, we adopt a conversion approach that transforms the PDDL representation into a more compact format while retaining critical syntactic information and reducing the token length. The compact form allows us to maintain the fidelity of the original PDDL files while making them suitable for fine-tuning LLMs with limited contextual length. Figure \ref{fig:pddl-vs-compact-ferry} illustrates the difference in token lengths between using PDDL and the compact data format for the \texttt{Ferry} domain as an example. We use plans in the same form without any modifications because their average token length for the dataset falls within the context length of LLMs. 

To evaluate the plan generation capabilities of the LLMs, we initially use datasets with identical distributions for training and testing, as shown in Figure \ref{fig:plantoken-ferry} for the \texttt{Ferry} domain. Additionally, we report the performance of LLMs on token lengths that fall outside the distribution of the training set.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/pddl-vs-compact-ferry.png}
    \caption{Token lengths for PDDL vs Compact Form}
    \label{fig:pddl-vs-compact-ferry}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/plantokens-ferry.png}
    \caption{Plan length distribution of of train and test sets}
    \label{fig:plantoken-ferry}
  \end{subfigure}
  \caption{(a) Token length for the \texttt{Ferry} domain. Using the PDDL compact form achieves an average 40\% reduction in token length in comparison to PDDL. (b) Plan length distribution is the same for train and test sets for initial analysis.}
  \label{fig:ferry-viz}
\end{figure}

\subsubsection{Data Format for Prompting}
To test LLMs capable of prompting \citep{brown2020language}, we directly use PDDL files as input as their context length is higher and also shows better performance than using the compact form. We adopt two prompting approaches, zero-shot, and few-shot, to test for planning capabilities in LLMs. In the zero-shot prompting approach, we provide the domain and problem files as input, without any additional examples, to evaluate the LLMs plan generation capabilities. In contrast, the few-shot prompting approach involves supplying a sample from the same domain and its corresponding plan in addition to the problem for which the LLM is required to generate plans. Through a comparative analysis of the fine-tuning and prompting approaches, we aim to provide insights into the effectiveness of LLMs and their potential for practical applications in planning scenarios.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
  \caption{LLM architectures used in our study.}
  \label{llm-arch}
  \centering
  \begin{tabular}{llllll}
    \toprule
    Model-Parameters & Pre-training & Layers & Heads & Embed. Size & Context Length\\
    \midrule
    T5-base-220M & NL & 12 & 12 & 768 & 512 \\
    CodeT5-base-220M & NL+code & 12 & 12 & 768 & 512 \\
    Codegen-multi-350M & NL+code & 24 & 16 & 1024 & 1024 \\
    text-davinci-03 & NL & NA & NA & NA & 8000 \\
    code-davinci-02 & NL+code & NA & NA & NA & 8000 \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Large Language Models: Overview and Considerations}

Table \ref{llm-arch} presents a comprehensive overview of the language models (LLMs) employed in this study, including critical design parameters such as the number of layers, heads, embedding size (head dimension), context length, and data source (natural language (NL) and/or code). Our investigation involves a combination of LLMs that have been pre-trained on natural language and code. Specifically, we utilize two OpenAI models, namely text-davinci-03 and code-davinci-02 for prompting with the temperature set to 0.2. Increasing the temperature value will result in the LLM being more creative and prone to taking risks. It is worth noting that both OpenAI models are derived from GPT-3, thereby inheriting its underlying architecture. However, the exact specifications of these models are unknown, and we leave this information as "not available" (NA) in our table. Our fine-tuning process involves T5, CodeT5, and Codegen models trained on the planning dataset using regularization and weight decay to prevent overfitting. We carry out our experiments using 24 CPU cores, along with a single A100 40GB GPU and 1TB of RAM. On average, the fine-tuning of each model takes less than 2.5 hours.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experimental Setup for Plan Generation}

In our study aimed at exploring the capabilities of LLMs in generating plans, we have formulated four research questions (RQ), each with its own set of corresponding metrics, in order to effectively address our research objectives. 

\noindent \textbf{RQ1:} \textbf{\textit{To what extent can LLMs solve planning problems?}}

Planning requires reasoning abilities, which involve generating a plan that satisfies given constraints. Recent research has demonstrated that pre-trained LLMs can reason in specific domains \citep{agrawal2023llms}. To answer how well pre-trained (or \textit{vanilla}) LLMs can generate plans, we test both state-of-the-art OpenAI models with zero-shot prompting and the others without fine-tuning. However, T5, CodeT5, and Codegen do not contain PDDL specification language as part of their training dataset and are expected to perform poorly without additional fine-tuning for domain adaptation. We employ a plan verification tool, VAL \citep{plan-verif-val}, to verify LLM-generated plans and evaluate them on planning-related metrics such as satisficing, optimal, invalid plans, and the degree of correctness.

\noindent \textbf{RQ2:} \textbf{\textit{What pre-training data is effective for plan generation?}}

After conducting experiments to address RQ1, we aim to provide a comprehensive response to the question of what pre-training data best suits LLMs in the context of plan generation. Specifically, we compare the performance of models pre-trained exclusively on textual corpora with those that incorporate both code and natural language during the pre-training process. Our ultimate goal is to provide a clear direction for future researchers to choose the appropriate LLMs, thereby advancing the field of LLM-based plan generation.

\noindent \textbf{RQ3:} \textbf{\textit{Which approach between fine-tuning and prompting improves plan generation?}}

Our objective is to compare the effectiveness of fine-tuning and prompting approaches for plan generation, specifically assessing whether updating model weights through fine-tuning provides superior domain adaptation compared to prompting LLMs for desired output. In addition to the experiments to address RQ1 and RQ2, we further explored the potential of T5, CodeT5, and Codegen models by fine-tuning them on the planning dataset with an 80\%-20\% train-test split. To complement our zero-shot prompting approach, we experimented with a few-shot prompting technique for text-davinci-03 and code-davinci-02. Using the same planning metrics as previously mentioned, we compared the results of the two approaches.

\noindent \textbf{RQ4:} \textbf{\textit{Are LLMs capable of plan generalization?}}

To the best of our knowledge, the current literature provides a limited understanding of the plan generalization capabilities of LLMs \citep{valmeekam2023planning}, as only a few studies have defined and quantitatively measured them.
To better evaluate the generalization capabilities of LLMs within the scope of planning we believe that the current definition of plan generalization needs to be revised due to its limited scope as it fails to account for all possible scenarios that may arise when using LLMs to plan. Therefore, we propose a new definition of plan generalization and introduce three new tasks to quantify the plan generalization capabilities of LLMs accurately.
This new definition can be then used to properly evaluate and categorize the various LLMs approaches.

%Moreover, the current definition of plan generalization needs to be revised due to its limited scope, thereby failing to account for all possible scenarios. Therefore, we propose a formal definition of plan generalization and introduce three new tasks to quantify the plan generalization capabilities of LLMs accurately. \todo[author = Vishal]{I think this paragraph is too blunt. Any modifications are helpful.}
\begin{definition}[Plan generalization capabilities of LLMs]
We define \emph{plan generalization capabilities of LLMs} as the ability to generate plans that are close to optimal plans for unseen, out-of-distribution problems from planning domains, where close is defined by a distance metric.
\end{definition}


%define m and n; averaged over the test set samples; ordering of the sentences to fit the formula
Let the training dataset be represented as $D_{train} = {(x_1, y_1), ..., (x_n, y_n)}$ where each $x_i$ is a planning problem and $y_i$ is the corresponding optimal plan for problem $x_i$. Let the testing dataset be represented as $D_{test} = {(x_{n+1}, y_{n+1}), ..., (x_m, y_m)}$ where each $x_i$ is a previously unseen planning problem and $y_i$ is the corresponding optimal plan for problem $x_i$. Note that $D_{train}$ and $D_{test}$ consist of pairs of planning problems and their corresponding optimal plans which are generated using FastDownward.

\begin{definition}[Plan generalization error]
    The plan generalization error is the average normalized hamming distance between the optimal plan and the LLM generated plan for each problem in $D_{test}$.
\end{definition}
 We use the Hamming distance between two plans to account for the differences in the order of actions. More formally, the plan generalization error $E_{pg}$ is defined as:

\begin{equation}
E_{pg} = \frac{1}{|m-n|} \sum_{i=n+1}^{m} \frac{H(y_i, \hat{y}_i)}{|A|}
\end{equation}

where $\hat{y}_i$ is the generated plan for $x_i \in D_{test}$, $H(\cdot,\cdot)$ is the Hamming distance between two plans, and $|A|$ is the total number of actions in the planning domain. A lower $E_{pg}$ means that LLM can produce plans more similar to the optimal plans generated by a traditional planning system. An LLM with $E_{pg}$ below a certain threshold (e.g., 0.5) is considered to have strong plan generalization capabilities. To evaluate the plan generalization capabilities of LLMs, we propose three tasks, which are defined formally below.

\noindent \textbf{\textit{Task 1:} Plan Length Generalization}
This task aims to evaluate the ability of LLMs to generalize to plan lengths that are outside the distribution of the training set. Given a set of planning domains belonging to the training set $\mathcal{D}={D_1, D_2, ..., D_n}$, we select a plan length $l_i$ for each domain $D_i$ that is outside the range of plan lengths in the training set. We then pose the planning problem for each domain with the selected plan length to the LLM. Let $\hat{\pi}$ denote the plan generated by the LLM, and let $\pi^*$ denote the optimal plan for the planning problem. We evaluate the plan $\hat{\pi}$ on planning-related metrics mentioned in RQ1 and also report $E_{pg}$.

\noindent \textbf{\textit{Task 2:} Object Name Randomization}
The second task involves testing the LLMs ability to generate plans using randomized object names not present in the training set. We first create a set of randomized object names for each planning domain in the dataset using the IPC problem generator. We then replace the object names in the planning problems in each domain for the test set with the randomized names. We pose the modified planning problems to the LLMs and evaluate the generated plan $\hat{\pi}$ using the planning metrics mentioned in Task 1.

\noindent \textbf{\textit{Task 3:} Unseen Domain Generalization}
The third task evaluates the LLMs ability to generalize to planning problems from new domains not included in the training set. We select a set of planning domains $\mathcal{D}'={D'_1, D'_2, ..., D'_m}$ that is disjointed from the training set. We pose the planning problems in each domain to the LLM and evaluate the generated plan $\hat{\pi}$ using the planning metrics mentioned in Task 1. 

Overall, we believe these tasks provide a comprehensive evaluation of the ability of LLMs to generalize to different types of planning problems.
